Fully Fluctuating Sleepy Consensus from Minimal Assumptions

Bitcoin's proof-of-work (PoW)-based protocol is remarkable for how little it asks of its participants. Not only can miners take breaks from work whenever they please, but it is almost unique in offering a path of contrition: corrupt miners can reclaim honest status simply by resuming mining on the longest chain. The protocol only requires that honest miners hold the majority of computational power at any given time. Analogous proof-of-stake (PoS) protocols, usually formalized via the sleepy model of Pass and Shi (2017), have fallen short of matching this robustness. In fact, sleepy consensus protocols in the plain PKI model must heavily restrict fluctuations in adversarial participation over time. The recent work of Efron, Neu, and Pitassi (2025) enables fully fluctuating participation in the sleepy model by introducing the external adversary model. Their protocol, however, relies on verifiable delay functions (VDFs), a strong cryptographic primitive that somewhat resembles PoW, by assuming that the adversary cannot compute sequential work significantly faster than honest nodes. In this work, we design a sleepy consensus protocol for fully fluctuating participation with an external adversary under an honest majority, from minimal assumptions: a public key infrastructure (PKI) and a verifiable random function (VRF). In particular, we make no VDF or hardware assumptions. Our key technique is graded wakeness, a novel primitive that allows nodes to form consistent opinions on which other nodes are awake. We further extend our protocol to handle uncorruption, where corrupt nodes return to honesty. This extension requires only a mild additional assumption on the unpredictability of VRF outputs for liveness.

==> floats/immobile_ba_gca2.tex <==
\begin{figure}[t]
    \centering
    \begin{tcolorbox}
        A node $p_i$ with input $x$ starts execution at round $0$ and executes the below steps at the start of the round $13v$ for every view $v \geq 0$.
        Beyond the outputs of $\gw$ and $\ga$, $p_i$ maintains the following state variables with the following initial values:
        \begin{itemize}
            \item \emph{Candidate: } $x_C \gets x$.
            \item \emph{Lock: } $x_L \gets \bot$.
        \end{itemize}

        \begin{protocolsteps}
            \item[$(t = 0 ... 12):$]Execute $\gca2_{v}$ with input $x_C$.
            \item[$(t = 12):$] If awake since the beginning of view $v$:\leavevmode
                  \begin{itemize}
                      \item Let $(x_L, g) \gets $ the output of $\gca2_{v}$.
                      \item If $g = 1$: output $x_L$.
                      \item Multicast $\signedproposemsg[i]{(x_L, \vrfo{v+1}, \pi)}$.
                  \end{itemize}
            \item[$(t = 13):$]\leavevmode 
                  \begin{itemize}
                      \item If $x_L = \bot$: set $x_{C} \gets $ the proposed value with the highest value VRF output for view $v + 1$; otherwise, set $x_{C} \gets x_{L}$.
                      \item If not awake since the beginning of the view: set $x_{C} \gets \noinput$.
                  \end{itemize}
        \end{protocolsteps}
        Note that $t = 13$ of view $v$ occurs alongside $t = 0$ of view $v + 1$.
    \end{tcolorbox}
    \caption{Byzantine agreement in the fully fluctuating sleepy model.}
    \label{fig:immobile-ba}
\end{figure}


==> floats/immobile_gca2.tex <==
\begin{figure}[t]
    \centering
    \begin{tcolorbox}
        A node $p_i$ with input $x$ executes the below steps starting from a round $t_s$.
        Let $t$ denote the rounds since $t_s$, where $t_s + t$ is the absolute round in the entire execution.
        \begin{protocolsteps}
            \item[$(t = 0 ... 6):$] Execute $\ga2_{0}$ with input $x$.
            \item[$(t = 6):$] Let $(y_0, g_0) \gets $ the output of $\ga2_{0}$ if it exists; otherwise, let $(y_0, g_0) \gets (\noinput, 0)$.
            \item[$(t = 6 ... 12):$] Execute $\ga2_{1}$ with input $y_0$.
            \item[$(t = 12):$] If awake since round $0$:\leavevmode
            \begin{itemize}
                \item Let $(y_1, g_1) \gets $ the output of $\ga2_{1}$.
                \item If $g_0 = 1$: output $(y_0, 1)$.
                \item Else if $g_1 = 1$: output $(y_1, 0)$.
                \item Otherwise, output $(\bot, 0)$.
            \end{itemize}
        \end{protocolsteps}
    \end{tcolorbox}
    \caption{Graded crusader agreement with $2$ grades for a node $p_i$.}
    \label{fig:immobile-gca2}
\end{figure}


==> lib/__hacks_floats.tex <==
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.8}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{0.8}
\renewcommand{\dbltopfraction}{0.9}
\renewcommand{\dblfloatpagefraction}{0.8}



==> lib/__hacks_spacing.tex <==
\setlength{\floatsep}{0.65\baselineskip}
\setlength{\textfloatsep}{1.15\baselineskip}
\setlength{\dblfloatsep}{0.65\baselineskip}
\setlength{\dbltextfloatsep}{1\baselineskip}

%
%
%
%

%
%
%
%

%
%

%
%
%
%
%
%
%
\widowpenalty=0
\clubpenalty=0
\brokenpenalty=0
%

\displaywidowpenalty=0
%
\setlength{\emergencystretch}{1em}   %

%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%


==> lib/defer.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\RequirePackage{expl3}
\RequirePackage{scontents}


%
%
%
\ExplSyntaxOn

%
%
%
\cs_new_protected:Npn \defer_new_group:nn #1 #2 {
  %
  \bool_if_exist:cF { l__defer_#1 _bool } { \bool_new:c { l__defer_#1 _bool } }
  %
  \tl_set:Nx \l_tmpa_tl { \tl_lower_case:n {#2} }
  %
  \str_if_eq:VnTF \l_tmpa_tl {deferred}
    { \bool_set_true:c  { l__defer_#1 _bool } }
    { \bool_set_false:c { l__defer_#1 _bool } }
}


%
%
%

%
%
\NewDocumentCommand{\newdefergroup}{m O{deferred}}{
  \defer_new_group:nn {#1}{#2}
}

%
%
\NewDocumentEnvironment{ifdeferred}{m +b}{%
  \bool_if:cT { l__defer_#1 _bool } { #2 }%
}{}

%
%
\NewDocumentEnvironment{ifnotdeferred}{m +b}{%
  \bool_if:cF { l__defer_#1 _bool } { #2 }%
}{}

%
%
%
\NewDocumentEnvironment{defer}{m +b}{%
  \bool_if:cTF { l__defer_#1 _bool }{%
    %
    \Scontents[store-cmd=defer@#1,print-cmd=false]{#2}%
  }{%
    %
    #2%
  }%
}{}

%
%
\NewDocumentCommand{\printdefergroup}{m}{%
  %
  \foreachsc{defer@#1}%
}

\ExplSyntaxOff

%
%
%

%
%
%
%
\NewDocumentCommand{\deferredproof}{m m}{%
  \begin{ifdeferred}{#1}%
    Proof of \cref{#2} is deferred to \cref{sec:deferred-#1}.%
  \end{ifdeferred}%
}

%
%
%
\NewDocumentCommand{\deferredsection}{m m}{%
  \begin{ifdeferred}{#1}%
    \section{#2}%
    \label{sec:deferred-#1}%
    \printdefergroup{#1}%
  \end{ifdeferred}%
}


==> lib/icons.tex <==
\usepackage{fontawesome5}
\usepackage{noto-emoji-easy}
\usepackage{tango-icons}


==> lib/tikzpgfplot.tex <==
\usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{fpu}
%
\usetikzlibrary{arrows.meta}
\usetikzlibrary{patterns}
\usetikzlibrary{positioning}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{calligraphy}
\usetikzlibrary{shapes.misc}
\usetikzlibrary{shapes.symbols}
\usetikzlibrary{shapes.arrows}
\usetikzlibrary{spy}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{intersections}
\usetikzlibrary{fit}


\usepackage{pgfplots}
\pgfplotsset{compat=1.18}
\usepgfplotslibrary{fillbetween}


\pgfplotsset{
    discard if not/.style 2 args={
            x filter/.code={
                    \edef\tempa{\thisrow{#1}}
                    \edef\tempb{#2}
                    \ifx\tempa\tempb
                    \else
                        \def\pgfmathresult{inf}
                    \fi
                }
        },
}



%

\pgfplotsset{
    mysimpleplot/.style = {
            %
            every axis plot/.prefix style={thick},
            %
            %
            width=1.05\linewidth,
            %
            height=0.75\linewidth,
            %
            %
            %
            %
            title style={font=\scriptsize,align=center},
            %
            %
            legend cell align=left,
            %
            legend style={font=\scriptsize},
            %
            legend columns=3,
            %
            %
            legend style={
                    at={(0.5,1)},
                    yshift=0.3em,
                    anchor=south,
                    draw=none,
                    /tikz/every even column/.append style={
                            column sep=0.3em
                        },
                    cells={
                            align=left
                        }
                },
            %
            grid=both,
            minor tick num=9,
            major grid style={solid,very thin,draw=gray!50},
            minor grid style={solid,ultra thin,draw=gray!20},
            %
            %
            %
            label style={font=\scriptsize,align=center},
            tick label style={font=\scriptsize},
            %
            %
        },
}

\pgfplotsset{
    mysimplefig1plot/.style = {
            mysimpleplot,
            xlabel={$\netX$},
            ylabel={$\tALident/n$},
            xmin=0.0, xmax=0.5,
            ymin=0.0, ymax=0.35,
            height=0.75\linewidth,
            width=\linewidth,
            yticklabel style={
                    /pgf/number format/fixed,
                    /pgf/number format/precision=2
                },
            scaled y ticks=false,
            %
            %
            xtick={0,0.1,0.2,0.25,0.33333,0.5},
            xticklabels={0,1/10,1/5,1/4,1/3,1/2},
            yticklabels={0,1/10,1/6,1/5,1/4,1/3},
            ytick={0,0.1,0.16666,0.2,0.25,0.33333},
        }
}




==> lib/tikzpgfplot_parulalinestyles.tex <==
\tikzset{myparula11/.style={color=myParula1Blue,solid,mark=+,mark options={solid}}}
\tikzset{myparula12/.style={color=myParula1Blue,densely dashed,mark=x,mark options={solid}}}
\tikzset{myparula13/.style={color=myParula1Blue,densely dotted,mark=o,mark options={solid}}}
\tikzset{myparula14/.style={color=myParula1Blue,dashdotted,mark=triangle,mark options={solid}}}
\tikzset{myparula15/.style={color=myParula1Blue,dashdotdotted,mark=square,mark options={solid}}}

\tikzset{myparula21/.style={color=myParula2Orange,solid,mark=+,mark options={solid}}}
\tikzset{myparula22/.style={color=myParula2Orange,densely dashed,mark=x,mark options={solid}}}
\tikzset{myparula23/.style={color=myParula2Orange,densely dotted,mark=o,mark options={solid}}}
\tikzset{myparula24/.style={color=myParula2Orange,dashdotted,mark=triangle,mark options={solid}}}
\tikzset{myparula25/.style={color=myParula2Orange,dashdotdotted,mark=square,mark options={solid}}}

\tikzset{myparula31/.style={color=myParula3Yellow,solid,mark=+,mark options={solid}}}
\tikzset{myparula32/.style={color=myParula3Yellow,densely dashed,mark=x,mark options={solid}}}
\tikzset{myparula33/.style={color=myParula3Yellow,densely dotted,mark=o,mark options={solid}}}
\tikzset{myparula34/.style={color=myParula3Yellow,dashdotted,mark=triangle,mark options={solid}}}
\tikzset{myparula35/.style={color=myParula3Yellow,dashdotdotted,mark=square,mark options={solid}}}

\tikzset{myparula41/.style={color=myParula4Purple,solid,mark=+,mark options={solid}}}
\tikzset{myparula42/.style={color=myParula4Purple,densely dashed,mark=x,mark options={solid}}}
\tikzset{myparula43/.style={color=myParula4Purple,densely dotted,mark=o,mark options={solid}}}
\tikzset{myparula44/.style={color=myParula4Purple,dashdotted,mark=triangle,mark options={solid}}}
\tikzset{myparula45/.style={color=myParula4Purple,dashdotdotted,mark=square,mark options={solid}}}

\tikzset{myparula51/.style={color=myParula5Green,solid,mark=+,mark options={solid}}}
\tikzset{myparula52/.style={color=myParula5Green,densely dashed,mark=x,mark options={solid}}}
\tikzset{myparula53/.style={color=myParula5Green,densely dotted,mark=o,mark options={solid}}}
\tikzset{myparula54/.style={color=myParula5Green,dashdotted,mark=triangle,mark options={solid}}}
\tikzset{myparula55/.style={color=myParula5Green,dashdotdotted,mark=square,mark options={solid}}}

\tikzset{myparula61/.style={color=myParula6LightBlue,solid,mark=+,mark options={solid}}}
\tikzset{myparula62/.style={color=myParula6LightBlue,densely dashed,mark=x,mark options={solid}}}
\tikzset{myparula63/.style={color=myParula6LightBlue,densely dotted,mark=o,mark options={solid}}}
\tikzset{myparula64/.style={color=myParula6LightBlue,dashdotted,mark=triangle,mark options={solid}}}
\tikzset{myparula65/.style={color=myParula6LightBlue,dashdotdotted,mark=square,mark options={solid}}}

\tikzset{myparula71/.style={color=myParula7Red,solid,mark=+,mark options={solid}}}
\tikzset{myparula72/.style={color=myParula7Red,densely dashed,mark=x,mark options={solid}}}
\tikzset{myparula73/.style={color=myParula7Red,densely dotted,mark=o,mark options={solid}}}
\tikzset{myparula74/.style={color=myParula7Red,dashdotted,mark=triangle,mark options={solid}}}
\tikzset{myparula75/.style={color=myParula7Red,dashdotdotted,mark=square,mark options={solid}}}



==> lib/utils.tex <==
\IfFileExists{version-string.txt}{%
  \newread\versionfile
  \openin\versionfile=version-string.txt
  \read\versionfile to \myVersionString
  \closein\versionfile
}{}
